Thermal state of the intergalactic medium at $z\sim2-4$

We present a new method to infer parameters of the temperature-density relation in the intergalactic medium in the post-reionization epoch at $z\sim 2-4$. This method is based on the analysis of the Ly$\alpha$ absorbers distribution over column densities and Doppler parameters by the model joint probability density function. This approach allows us to measure the power-law index $\gamma$ of the temperature-density relation and a certain combination of the temperature at the mean density $T_0$ and hydrogen photoionization rate $\Gamma$. To estimate $T_0$ and $\Gamma$ separately, we employ measurements of the Ly$\alpha$ forest effective opacity and the model gas probability density function. We show that $\gamma$ tends to be lower than 1.6 and reaches 1.3 at redshift $\sim3$. The inferred temperatures at the mean density are $\sim(2\pm0.5)\times10^4$ K in the studied redshift range. Both these estimates favour HeII reionization at $z\gtrsim3$. We find that the hydrogen photoionization rate is $\sim0.6\times10^{-12}$ s$^{-1}$, which is consistent with previous measurements.

==> journals.tex <==
\def\apj{Astroph. J.}
\def\apjl{Astroph. J. Lett.}
\def\apjs{Astroph. J. Suppl.}
%\def\mnras{Mon. Not. Roy. Astron. Soc.}
\def\mnras{MNRAS}
\def\nat{Nature}
\def\aap{Astron. Astroph.}
\def\pr{Phys. Rev.}
\def\pra{Phys. Rev. {\rm A}}
\def\prc{Phys. Rev. {\rm C}}
\def\prb{Phys. Rev. {\rm B}}
\def\prd{Phys. Rev. {\rm D}}
\def\prl{Phys. Rev. Lett.}
\def\plb{Physics Letters {\rm B}}
\def\apss{Astroph. Space Sci.}
\def\pla{Physics Letters {\rm A}}
\def\ssr{Space Sci. Rev.}
\def\araa{Ann. Rev. Astron. Astroph.}
\def\aj{Astron. J.}
\def\pasp{Pub. Astron. Soc. Pacific}
\def\memras{Mem. R. Astron. Soc.}
\def\jpcs{J. Phys.: Conf. Ser.}
